Factorize Factorization

Factorization -- a simple form of standardization -- is concerned with reduction strategies, i.e. how a result is computed. We present a new technique for proving factorization theorems for compound rewriting systems in a modular way, which is inspired by the Hindley-Rosen technique for confluence. Specifically, our technique is well adapted to deal with extensions of the call-by-name and call-by-value lambda-calculi. The technique is first developed abstractly. We isolate a sufficient condition (called linear swap) for lifting factorization from components to the compound system, and which is compatible with beta-reduction. We then closely analyze some common factorization schemas for the lambda-calculus. Concretely, we apply our technique to diverse extensions of the lambda-calculus, among which de' Liguoro and Piperno's non-deterministic lambda-calculus and -- for call-by-value -- Carraro and Guerrieri's shuffling calculus. For both calculi the literature contains factorization theorems. In both cases, we give a new proof which is neat, simpler than the original, and strikingly shorter.

==> 03-modular.tex <==
% !TEX root = main_modular.tex
\section{Modularizing Factorization}\label{sec:modular}
%\subsubsection{Factorization via Local Postponement and a  Mediating Relation.}








\begin{definition}[LOcal Postponement Pair  (LOPP)]\label{def:slop}
	A pair $(A,\{\ereda,  \ireda\})$ and  $(A,\{\eredc,  \iredc\})$   of ARS form a  LOPP if the 
following conditions hold, where  $\eredx{} ~=~\ereda \cup \eredc$

%\begin{center}
{ 		\begin{tabular}{lll}\centering
		\textsf{Local Postponement of $\reda$}:&\quad\quad& $\ireda \cdot \ereda$ implies  $\ereda^*\cdot  
\ireda^=$\\
		\textsf{Local Postponement of $\redc$}:& &$\iredc  \cdot \eredc$ implies  $\eredc^*\cdot  
\iredc^=$,\\
		\textsf{Swap  of $\ireda$ after  $\eredc$:} & &$\ireda \cdot \eredc$ implies  $\eredx{}^*\cdot  
\ireda^=$,\\
		\textsf{Swap of $\iredc$ after  $\ereda$:}  && $\iredc  \cdot \ereda$ implies  $\eredx{}^*\cdot  
\iredc^=$.\\
	\end{tabular}}
%\end{center}
%	\begin{enumerate}
%		\item \emph{Local Postponement of $\reda$}:\quad $\LP{\ereda}{\ireda}$,  
%		\item \emph{Local Postponement of $\redc$}:\quad $\LP{\eredc}{\iredc}$,
%		\item $\Swap{}{} $ of $\ireda$:\quad $\ireda \cdot \eredc$ implies  $\ered^*\cdot  \ireda$,	
%		\item 	$\Swap{} {}$ of $\iredc$:  \quad $\iredc  \cdot \ereda$ implies  $\ered^*\cdot  \iredc$;
%	\end{enumerate}
%
\end{definition}
Note $\ered$ in  the right-hand side of the \swap conditions.
%Note that  on the r.h.s. of the \swap condition $\ered ~=~\ereda \cup \eredc$.
The four conditions  essentially say that $\ireda$ postpones \emph{after both} $\ereda$ and 
$\eredc$, and similarly for  $\iredc$. 
 

 

	\begin{remark}
	The four  conditions above can   be  unified in  following compact  condition:
	\begin{center}
		$\iredx{\tau } \cdot \eredx{\rho}$ implies  $\eredx{\rho\tau}^*\cdot \iredx{\tau}^=$ for all $\tau , \rho 
\in \set{\alpha,\gamma}$. 
	\end{center}
The condition, and the  result below, easily extends to the union of \emph{any number of relations}
\end{remark}

\begin{lemma}[]\label{l:modularity} 
	If  $(A,\{\ereda,  \ireda\})$ and  $(A,\{\eredc,  \iredc\})$ form  a LOPP, then   their union 
satisfies \emph{local postponement} $\LP{\ered}{\ired}$, where $\ired \,\defeq\, (\ireda 
\cup\iredc)$ and $\ered \ \defeq \ (\ereda \cup\eredc)$.
\end{lemma}

\begin{proof}
%	For local postponement, we show $\ired \ered$ implies  $\ered^*  \ired  $ by simply verifying the 
%4 combinations of $\ired \ered$ 
It is immediate that $\ired \cdot \ered$ implies  $\ered^* \cdot \ired^=  $, because  the 4 combinations of 
$\ired \cdot \ered$ ($\ireda\cdot\ereda,  ~\iredc \cdot\eredc, ~ \ireda \cdot\eredc, ~ \iredc \cdot\ereda$) exactly 
  correspond to the 4 conditions.
\SLV{}{	\begin{itemize}
		\item $\ireda\ereda$ implies  $\ered^*  \ired  $  by  local postponement  for $\reda$,
		\item $\iredc\eredc$ implies  $\ered^*  \ired  $ by  local postponement  for $\redc$,
		\item $\ireda\eredc$ implies $\ered^*  \ired  $ by   \swap  of $\ireda$,
		\item $\iredc\ereda$ implies $\ered^*  \ired  $ by   \swap of $\iredc$.
	\end{itemize}}
\end{proof}


	Let  $\reda ~= ~\ereda \cup \ireda$ and $\redc ~= ~\eredc \cup \iredc$ be  $\ex$-factorizing relations.
Then their union  $\reda \cup \redb$ satisfies 
factorization
$\F\ired\ered$,  where  $\ired \,\defeq\, (\ireda \cup\iredc)$ and $\ered \ \defeq \ (\ereda 
\cup\eredc)$.

	 
In this section, we set 	 
 \begin{itemize}
 	\item $\reda ~= ~\ereda \cup \ireda$ and $\redc ~= ~\eredc \cup \iredc$.

\item   $\ired \,\defeq\, (\ireda \cup\iredc)$ and $\ered \ \defeq \ (\ereda    \cup\eredc)$.

 \end{itemize}

\begin{lemma}\label{thm:modularityM} 
	Assume  that   $\reda ~= ~\ereda \cup \ireda$ and $\redc ~= ~\eredc \cup \iredc$ are   $\ex$-factorizing relations, and that 
\begin{center}
		$\ireda^* \cdot \eredc   \subseteq (\ereda \cup \eredc)^*\cdot  
		\ireda^*$ \quad and \quad 
		 $\iredc^*  \cdot \ereda \subseteq {(\ereda \cup \eredc)}^*\cdot  
		\iredc^*$.
\end{center}
Then the following hold
\begin{enumerate}
	\item $\PP{\ereda \cup \eredc}{\ireda^* \cup \iredc^*}$
	\item 	$\PP{\ereda \cup \eredc}{\ireda \cup \iredc}$
\end{enumerate}		

	
\end{lemma}

\begin{proof} \begin{enumerate}
		\item follows immediately from the observation that  $\LP{ \ereda \cup \eredc}{\ireda^* \cup \iredc^*}$ 
		 holds, because the assumptions give exactly the  four combinations
		$\iredx k \cdot \eredx{j}$ , for $k,j\in \{\alpha,\gamma\}$.
		\item  follows from (1.) by  \reflemma{characterization}
	\end{enumerate}
\end{proof}

\RED{
\begin{lemma}\label{thm:modularityM} 
Assume  that   $\reda ~= ~\ereda \cup \ireda$ and $\redc ~= ~\eredc \cup \iredc$ are   $\ex$-factorizing relations, and that 

	\begin{tabular}{ll}
	%	\textsf{Swap  of $\ireda$ after  $\eredc$:} 
	 &$\iparreda \cdot \eredc$ implies  $(\ereda \cup \eredc)^*\cdot  
		\iparreda^=$.\\
	%	\textsf{Swap of $\iredc$ after  $\ereda$:} 
		 & $\iparredc  \cdot \ereda$ implies  ${(\ereda \cup \eredc)}^*\cdot  
		\iparredc^=$.\\
	\end{tabular}
	for some $\iparreda, \iparredc$ such that  $\iparreda^*=\ireda^*$ and $\iparredc^*=\iredc^*$.

Then the following hold
\begin{enumerate}
	\item $\F{\ereda \cup \eredc}{\iparreda \cup \iparredc}$
	\item 	$\F{\ereda \cup \eredc}{\ireda \cup \iredc}$
\end{enumerate}	
\end{lemma}

\begin{proof} 
	\begin{enumerate}
		\item follows immediately from the observation that  $\LP{ \ereda \cup \eredc}{\iparreda \cup \iparredc} $ holds, because the assumptions give the  four combinations
		$\iparred_j \cdot \eredx{k}$. 
		\item  follows from (1.) by  \reflemma{characterization}, where we instantiate $\iparred := (\iparreda \cup \iparredc)$. Note that $ (\iparreda \cup \iparredc)^* ~=~ (\ireda\cup \iredc)^*$,   by the assumptions  and property \refeq{eq:closure_U} (page \pageref{eq:closure_U}).
	\end{enumerate}

	\end{proof}}




\subsection{Union of Factorizing Relations}
We formulated \refthm{modularityM} in full generality; this  allows for $\parred$ to be any mediating relation we need, for example a parallel reduction.
We now focus on a specific choice and provide a simple \emph{local} diagram implying the 
swap conditions. 

 Since we want to study under which conditions the union $\reda\cup\redc$ of factorizing relations  
satisfies factorization,  the  most natural choice is to take directly  $\iparreda:=\ireda^*$ and 
$\iparredc:=\iredc^*$.
Assuming that $\reda$ and $\redc$ factorize separately,  by   \refthm{modularityM}, we have that  
the following are sufficient conditions to guarantee that $\reda\cup\redc$ factorizes  (note that  local postponement of $\ireda^*$ and$  \iredc^* $ is given  by \refl{characterization}):
\begin{center}
		\small{ 	\textsf{Swap of $\ireda^*$  after $\eredc$:}~~	 	$ \ireda^* \cdot \eredc  \subseteq \ered^* \cdot \ireda^*$~~ {and} ~~  
		\textsf{Swap of $\iredc^*$  after $\ereda$:} ~~	 $ 	\iredc^* \cdot \ereda \subseteq  \ered^* \cdot\iredc^* $.}
\end{center}
These    conditions are  rather strong, because  global, hence  difficult to verify. 
Perhaps surprisingly, the following easy-to-check condition, which is \emph{local} and 
\emph{linear} in $\ered$, suffices, and  holds  in a large variety of cases. Note $\reda^*$ in the right-hand side. We say that $\ireda$ 
\textbf{linearly swaps} with $\eredc$ if
\begin{equation}\label{eq:LS}\tag{\textbf{Linear Swap}}\centering
	\LS\ireda\eredc:~~\ireda \cdot   \eredc  \ \subseteq\  \eredc \cdot \reda^*
\end{equation}

%
\begin{lemma}[Linear Swap] \label{l:simple_swap} 
%If	$\F\ereda\ireda$ and $\LS\ireda\eredc$ then ( $\ireda^*$ swaps after $\eredc$).
%If $\F\ereda\ireda$, then  ($\ireda^*$ swaps after $\eredc$) if		$\LS\ireda\eredc$.
$\F\ereda\ireda$ and $\LS\ireda\eredc$ $\implies$ (\textsf{Swap of $\ireda^*$ after $\eredc$}).
\end{lemma}
\begin{proof} $\LS\ireda\eredc$ implies 
	$(\ireda)^* \cdot \eredc$ $\subseteq$  $\eredc \cdot\reda^*$, by   \reffact{basic_com}. 
	By factorization of $\reda$, we obtain $(\ireda)^* \cdot \eredc$ $\subseteq$  $\eredc \cdot \ereda^* \cdot\ireda^*$.
\end{proof}
%


By  \refthm{modularityM} and \reflem{simple_swap}, we obtain  that the union of two  factorizing 
relations $\reda$, $\redc$ is factorizing if two elementary  conditions are verified.
\begin{cor}[Modular Factorization, linearly]\label{cor:HR_modularity}
	Let  $\reda ~= ~(\ereda \cup \ireda)$ and $\redc ~= ~(\eredc \cup \iredc)$ be  $\ex$-factorizing relations, such that 
%	\begin{center}
%		$\LS\ireda\eredc$ ~~and~~ $\LS\iredc\ereda$.
%	\end{center}
\begin{center}
		$\LS\ireda \eredc:~~\ireda \cdot \eredc$ $\subseteq$  $\eredc \cdot \reda^*$ \quad and \quad
		$\LS\iredc \ereda:~~\iredc \cdot \ereda$ $\subseteq$  $\ereda \cdot \redc^*$.
\end{center}
%	\begin{align*}
%	\ireda \, \eredc \ &\subseteq \ \eredc \, \reda^* 
%	& \text{and} &&
%	\iredc \, \ereda \ \subseteq \ \ereda \, \redc^*.
%	\end{align*}
	Then 	their union
	$\reda\cup \redc$  satisfies 
		$\F{\ered}{\ired}$
		where   $\ered \ := \ \ereda \cup\eredc$, and $\ired \ := \ \ireda \cup\iredc$. 

	
\end{cor}

%In \refsec{studies} we apply this result to several concrete cases of calculi which extend or refine $\lam$-calculus.
\paragraph*{Linear Postponement.}
The  idea behind the linear swap condition also applies to local postponement. The following   will 
simplify the proof of factorization in several  of our case studies.
%We conclude this section by stating two properties which  allow us to simplify the proof of factorization in many cases.

\begin{lemma}[Linear postponement]\label{l:easy_lp} Let $\red~=~\{\ered,\ired\}$
	\begin{enumerate}
		
		\item	($\ired \cdot \ered ~\subseteq~ \ered \cdot \ired^*)   ~\Rightarrow~ \LP{\ered}{\ired^*}   ~\Rightarrow~ \F{\ered}{\ired}$.
		
			\item 	($\ired  \cdot  \ered ~ \subseteq ~\ered  \cdot \red^= )  ~\Rightarrow~ \LP{\ered}{\ired} ~\Rightarrow~ \F{\ered}{\ired}$.
	\end{enumerate}
\end{lemma}

\SLV{}{
	Finally, observe that
	\begin{remark}  
		$\LP{\ered}{\ired}$ 
		can equivalently be written as 
		$\ired  \cdot  \ered ~ \subseteq ~\ered^*  \cdot \red^= $
		
	\end{remark} 
}


%%%%%%%%%%%%%%%%%
	
	
	
\condinc{}{
	Clearly, $\iparreda^*=\ireda^*$ (trivially) and $\LP{\ereda}{\ireda^*}$ (by \reflemma{characterization}).  We only need to check that 
\begin{center}
	$\ireda^*$ swaps after $\eredc$
\end{center}
that is
\begin{center}
$\#:$~~	$\ireda^*$ $\eredc$ $\subseteq$  $\ered^* ~\ireda^*$.
\end{center}
%	

A simplification is immediately possible, which makes inductive proofs  easier (note $\reda^*$ instead of $\ireda^*$)
\begin{lemma}[ Swap] \label{l:swap}If $\F\ereda\ireda$, then 
	\begin{center}
		$\ireda^*$ $\eredc$ $\subseteq$  $\eredc^*~\reda^*$
	\end{center}
	implies 
	that $\ireda^*$ swaps after  $\eredc$.
\end{lemma}

\begin{proof} 
	 By factorization of $\reda$, we obtain 
	$(\ireda)^*$ $\eredc$ $\subseteq$  $\eredc~\ereda^*~\ireda^*$.
\end{proof}
This  condition   is still  rather strong, as it is universally quantified on  sequences of $\ireda$ steps,  and therefore it may be difficult to verify in practice. 
%
Let us define a local condition of swap, which is \emph{linear}  in $\ered$. We say that $\ireda$ \textbf{linearly swaps} with $\eredc$ if
\begin{center}
	$\LS\ireda\eredc:~~\ireda$ $\eredc$ $\subseteq$  $\eredc ~\reda^*$
\end{center}
 This simple, efficient  condition is sufficient  to establish $\#$; perhaps surprisingly, it hold in a large variety of cases.
 
 

 
 
\begin{lemma}[Linear Swap] \label{l:simple_swap}If $\F\ereda\ireda$, then  $\ireda^*$ swaps after $\eredc$ if
\begin{center}
	$\LS\ireda\eredc:~~\ireda$ $\eredc$ $\subseteq$  $\eredc ~\reda^*$
\end{center}
\end{lemma}
\begin{proof} 
	 $(\ireda)^*$ $\eredc$ $\subseteq$  $\eredc~\reda^*$, by   \reffact{basic_com}. 
	 %By factorization of $\reda$, we obtain $(\ireda)^*$ $\eredc$ $\subseteq$  $\eredc~\ereda^*~\ireda^*$.
\end{proof}
%


We therefore have that the union of two  factorizing relations $\reda$, $\redc$ is factorizing if a simple swap condition is verified
\begin{cor}[Modular Factorization, linearly]\label{cor:HR_modularity}
Let  $\reda ~= ~\ereda \cup \ireda$ and $\redc ~= ~\eredc \cup \iredc$ be  $\ex$-factorizing relations, such that 
\begin{align*}
	\ireda \, \eredc \ &\subseteq \ \eredc \, \reda^* 
	& \text{and} &&
	\iredc \, \ereda \ \subseteq \ \ereda \, \redc^*.
\end{align*}
	  Then 	their union
	 	$\reda\cup \redc$  satisfies 
	\begin{center}
			$\F{\ered}{\ired}$
 where   $\ered \eq \ereda \cup\eredc$, and $\ired\eq\ireda \cup\iredc$. 
	\end{center}

\end{cor}
 
In \refsec{studies} we apply this result to several concrete cases of calculi which extend or refine $\lam$-calculus.
}


%
%\paragraph*{Discussion: $\lam$-calculus?}	In the next section, we apply our 
%method to study factorization in several extensions of $\lam$-calculus. 		Perhaps surprisingly, we can use   \refcor{HR_modularity} directly, without need for to define  a notion of parallel reduction involving the new rules. 
%
%
%	This is remarkable, since in the $\lam$-calculus, the role of a mediating relation is typically played by parallel reduction (see Remark at page \pageref{rem:parallel}). 

	


==> 06-conclusion.tex <==
% !TEX root = main_modular.tex
	\section{Conclusion}
		
We have observed  that the relation between Factorization and Local Postponement is similar to the most famous relation between Confluence and the Diamond property, as summarized in the following table
\begin{center}
	\begin{tabular}{l|l|l|l}
&global:&	\textbf{Confluence} & \textbf{Factorization}\\

&local:&	\textbf{Diamond} & \textbf{Local Postponement}\\
\hline
1.&& ($ \red $ confluent) $ \Leftrightarrow $  ($\red^*$ diamond)~~ & $\F{\ered}{\ired}$ $ \Leftrightarrow $ 	$\LP{\ered} {\ired^*}$\\
2.& & \reflemma{diamonds} & \reflemma{characterization} \\

3. &from line (2):&Tait and Martin-L\"of method  & Takahashi method\\
&&(based on Parallel Reduction)&(based on Parallel Reductions)\\
4. & from line (2):&   Hindley-Rosen method  & ~~~\textbf{		???}\\
\end{tabular}
\end{center}
In this paper, we have filled the ??? gap in the last line.



		
		\subsection{Limits and future work.}
		
		\input{99future}
